A Structure-Preserving Semi-Lagrangian based bi-fidelity method for the Vlasov--Poisson system with uncertainties

Uncertainty quantification for the Vlasov--Poisson (VP) systems entails repeated dynamic simulations, incurring immense computational costs. We develop a structure-preserving Semi-Lagrangian (SL) b-fidelity approximation of macroscopic observables. The MUSCL is used as a low-fidelity solver for pressureless Euler--Poisson system, allowing for a more cost-effective exploration of the stochastic parameter space. A conservative SL scheme combined with high-order discontinuous Galerkin is used as a high-fidelity solver for collisionless VP system, whose mass conservation, positivity preservation, and low numerical dissipation provide a more reliable high-fidelity snapshots for bi-fidelity reconstruction. We further derive a conditional error bound that separates projection, discretization, and model errors. Numerical experiments for both deterministic and uncertain VP problems, including multispecies and higher-dimensional settings, demonstrate that the proposed framework achieves accurate and robust uncertainty propagation.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamremark{fact}{Fact}
\crefname{fact}{Fact}{Facts}

% Sets running headers as well as PDF title and authors
\headers{SL Bi-Fidelity for uncertain VP}{X. Cai, J. Guo, and L. Liu}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{A Structure-Preserving Semi-Lagrangian based bi-fidelity method for the Vlasov--Poisson system with uncertainties\thanks{Submitted to the editors October 16, 2026.
\funding{The work of the third author was supported by  the National Key R\&D Program of China (2021YFA1001200), the Ministry of Science and Technology of China, the General Research Fund of the Research Grants Council of Hong Kong (14303022, 14301423, 14307125, 14310726).
The work of the first author and the second author was partially supported by the NSFC (No 12671463), Guangdong basic and applied basic research foundation [2025A1515012182], Guangdong and Hong Kong Universities “1+1+1” Joint Research Collaboration Scheme [2025A0505000014].}}}

% Authors: full names plus addresses.
\author{
  Xiaofeng Cai\thanks{Department of Mathematics, Faculty of Arts and Sciences, Beijing Normal University, Zhuhai,
519087, P.R. China (\email{xfcai@bnu.edu.cn}).}
  \and
  Jiaojiao Guo\thanks{Department of Mathematics, Faculty of Arts and Sciences, Beijing Normal University, Zhuhai,
519087, P.R. China (\email{gjiaojiao@mail.bnu.edu.cn}).}
  \and
  Liu Liu\thanks{The Chinese University of Hong Kong, Hong Kong (\email{lliu@math.cuhk.edu.hk}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> title.tex <==
% 论文标题
\title{A conservative semi-Lagrangian based bi-fidelity method for the Vlasov-Poisson system with uncertainties}

% 作者1 (通讯作者)
\author[inst1]{Xiaofeng Cai}%

% 其他作者
\author[inst1]{Jiaojiao Guo}%
\author[inst2]{Liu Liu\corref{cor1}}%
\ead{email@university.edu}
\cortext[cor1]{Corresponding author}

% 机构信息
\affiliation[inst1]{organization={Department Name, University Name},
            addressline={Street Address}, 
            city={City},
            postcode={000000}, 
            country={China}}

\affiliation[inst2]{organization={Department Name, University Name},
            addressline={Street Address}, 
            city={City},
            postcode={000000}, 
            country={China}}
            
\affiliation[inst3]{organization={Research Lab Name},
            city={City},
            country={*}}



% 摘要
\begin{abstract}
%在这里输入你的摘要内容。
\end{abstract}

% 关键词
\begin{keyword}
Keyword 1 \sep Keyword 2 \sep Keyword 3
\end{keyword}
